Clock Auctions Augmented with Unreliable Advice

We provide the first analysis of (deferred acceptance) clock auctions in the learning-augmented framework. These auctions satisfy a unique list of appealing properties, including obvious strategyproofness, transparency, and unconditional winner privacy, making them particularly well-suited for real-world applications. However, early work that evaluated their performance from a worst-case analysis perspective concluded that no deterministic clock auction with $n$ bidders can achieve a $O(\log^{1-\epsilon} n)$ approximation of the optimal social welfare for any $\epsilon>0$, even in very simple settings. This overly pessimistic impossibility result heavily depends on the assumption that the designer has no information regarding the bidders' values. Leveraging the learning-augmented framework, we instead consider a designer equipped with some (machine-learned) advice regarding the optimal solution; this advice can provide useful guidance if accurate, but it may be unreliable. Our main results are learning-augmented clock auctions that use this advice to achieve much stronger guarantees whenever the advice is accurate (consistency), while maintaining worst-case guarantees even if this advice is arbitrarily inaccurate (robustness). Our first clock auction achieves the best of both worlds: $(1+\epsilon)$-consistency for any $\epsilon>0$ and $O(\log{n})$ robustness; we also extend this auction to achieve error tolerance. We then consider a much stronger notion of consistency, which we refer to as consistency$^\infty$, and provide auctions that achieves a near-optimal trade-off between consistency$^\infty$ and robustness. Finally, using our impossibility results regarding this trade-off, we prove lower bounds on the ``cost of smoothness,'' i.e., on the achievable robustness if we also require that the performance of the auction degrades smoothly as a function of the prediction error.

==> 36-consistencytau.tex <==
% \begin{enumerate}
%     \item notion of smoothness
%         \begin{enumerate}
%             \item unifying error definition
%             \item linear smooth being the standard guarantee people aim for
%         \end{enumerate}

%     \item Spectrum of smoothness
%         \begin{enumerate}
%             \item with error-tolerance type of results being an example
%         \end{enumerate}

%     \item \tconsistency: the unifying definition, consistency$^1$, \sconsistency being two extreme point
% \end{enumerate}

An important shortcoming of the standard consistency measure is that it only binds when the prediction is perfectly accurate; it provides no performance guarantees when the prediction is inaccurate, even if the prediction error is very small. To overcome this issue, an important goal is to also achieve \emph{smoothness}, i.e., some performance guarantees that bind even if the prediction is not fully accurate. 


One way to achieve this smoothness is to provide a guarantee that is always close to the best solution if the given predictions are correct.
To this end, we consider a stronger notion of consistency first proposed by \cite{MNS07}, which we 
denote as \sconsistency. It is defined to be the worst-case approximation ratio with respect to \emph{the value of the predicted set}, regardless of the correctness of the prediction. We provide below a definition for general learning-augmented algorithm design problem.
\begin{definition}[\sconsistency] Given some maximization problem with objective function $f(\cdot)$. Given an instance $I$, let $\gpred$ denote the predictions.  Let $\texttt{ALG}_{\gpred}$ be the optimal algorithm for the problem, assuming the prediction is correct. The \sconsistency\ of a given algorithm \texttt{ALG}(I, $\gpred$) is defined as:
\[\text{\sconsistency}(\texttt{ALG}) = \max_{I, \gpred} \frac{f(\texttt{ALG}_{\gpred}(I))}{f(\texttt{ALG}(I, \gpred))}.\]
\end{definition}
As an example, in our setting, where the prediction is the predicted optimal set $\pred$, the \sconsistency\ of any mechanism $\mech$ is defined as: 
\begin{align}\label{def:consistency2}
    \text{\sconsistency}(\mech) = \max_{I, \pred} \frac{v(\pred)}{\mech(I, \pred)},
\end{align}
Since if the prediction is accurate, the best algorithm would outputs the predicted set as the maximum value set.
we emphasize that an $\alpha$-\sconsistency\ guarantee implies an $\alpha$-consistency guarantee for any $\alpha$ by considering a subset of instances where $\pred = \opt(I)$. If some mechanism achieves $\alpha$-\sconsistency, then it achieves an approximation of $\alpha \cdot \frac{v(\opt)}{v(\pred)}$, where $\frac{v(\opt)}{v(\pred)}$ captures the error of the prediction in terms of the performance. 

\paragraph{A universal definition of error.} We now introduce a general error definition applicable to any learning-augmented algorithm design problem. Broadly, this definition aims to quantify the performance loss—whether in terms of approximation ratio, runtime, complexity, etc.—when treating the prediction as if it were accurate. Specifically, if the prediction is indeed correct, the error would be 1, whereas an arbitrary prediction may result in unbounded error. Unlike other error definitions in the literature, which focus more on the statistical or learning characteristics of predictions, this error definition is based on its impact on the performance of the given problem and objective functions. Formally

\begin{definition}[performance-based error]For a given  minimization problem, let $f(A)$ be the objective function given an outcome $A$. Given an instance $I$, let $\gpred$ denote the predictions and $\opt(I)$ be the optimal outcome of the given instance w.r.t the performance function $f$.  Let $\texttt{ALG}_{\gpred}$ be the optimal algorithm for the problem, assuming the prediction is correct. The \emph{error} of a prediction with respect to instance $I$ is defined to be:
\[\eta\left(I, \gpred\right)= \frac{f(\opt(I))}{f(\texttt{ALG}_{\gpred}(I))}.\]
\end{definition}
For example, in our setting, where the prediction is the predicted optimal set $\pred$, the error of the predictions is the multiplicative difference between the value of the predicted set and the value of the optimal set, i.e., 
\begin{align}\label{def:error}
    \eta(\pred, I) = \frac{v(\opt(I))}{v(\pred)}.
\end{align}
This is because, assuming the prediction is accurate, the best algorithm outputs the predicted set as the maximum-value set. In settings where the prediction is the entire instance $\hat{I}$, the best algorithm, $\texttt{ALG}_{\hat{I}}$, would be the optimal algorithm for the full-information (or offline) version of instance $\hat{I}$. This error definition is commonly used in the literature \textcolor{blue}{add cite}, though it is not always explicitly defined.

% Another desired guarantee in the literature is good performance as a function of the error. Given a performance-based error, this is straightforward to achieve: simply run the optimal algorithm assuming the prediction is correct. By definition, such an algorithm would achieve a performance guarantee of $\eta$. The real challenge, however, lies in obtaining both good performance as a function of the error—referred to here as \emph{smoothness}—as well as robustness. To address this, we turn to a stronger consistency definition, namely, \sconsistency. Recall that \sconsistency\ is defined as the worst-case approximation ratio with respect to the value of the predicted set, regardless of prediction accuracy. Mathematically,
% \[
%     \text{\sconsistency}(\mech) = \max_{I, \pred} \frac{v(\pred)}{\mech(I, \pred)}.
% \]

Given a performance-based error, we can translate between the \sconsistency\  notion and the smoothness notion. For upper bounds, note that if a mechanism is $\alpha$-consistent with $\beta$-robustness, it achieves an $\alpha\eta$ approximation, where $\eta$ is the performance-based error, with $\beta$-robustness. For constant $\alpha$, this performance scales linearly with the error, which is often the desired error dependency in the literature. Importantly, for lower bounds, an impossibility result on the trade-off between $\alpha$-\sconsistency\ and robustness implies an impossibility result for achieving $\alpha \eta$ performance and robustness. To our knowledge, no prior work provides explicit impossibility results on the trade-off between error-dependence and robustness. In the next section, we provide matching upper and lower bounds for this trade-off, establishing the first such impossibility result.

\paragraph{Capped Smoothness}Such a strong dependence on error may not always be desirable, especially if the cost of achieving such smoothness results in inadequate robustness. Ideally, a mechanism should allow flexibility in choosing the extent of good error-dependence, enabling a balance between smoothness and robustness. To address this, we introduce a spectrum of consistency notions that generalizes both standard consistency and \sconsistency\ and interpolates between them.

\begin{definition}[\tconsistency]
Given a parameter $\tau \geq 1$, the \tconsistency\ is defined as the worst-case approximation ratio with respect to the value of the predicted set, for any instance where the performance-based error is less than $\tau$. Formally,
\[
\text{\tconsistency}(\mech) = \max_{I, \pred: \eta\left(I, \pred\right) \leq \tau} \frac{v(\opt)}{M(I, \pred)}.
\]
\end{definition}

Note that consistency$^1$ corresponds to the standard notion of consistency.

As an example, we introduce the \errmech\ auction, which extends Mechanism~\ref{alg:follow-the-leader}. This auction accepts a parameter $\tau \geq 1$, called the smoothness cap, which the mechanism designer can adjust. The only modification from Mechanism~\ref{alg:follow-the-leader} to \errmech\ is that in Line~\ref{alg:line:Prevc}, the targeted revenue is adjusted from $R_t$ to $R_t/\tau$. When the prediction error $\eta$ is at most $\tau$, \errmech\ achieves an approximation of $(1+\epsilon)\eta$ to the optimal welfare. Additionally, it maintains an approximation of $\left(\frac{2000\tau(1+\epsilon)}{9\epsilon}+1\right)H_n$ to the optimal welfare at all times. If $\tau = 1$, the auction defaults to Mechanism~\ref{alg:follow-the-leader}, retaining the corresponding consistency and robustness guarantees. The formal description of \errmech\ and the proof of the following theorem are deferred to Appendix~\ref{app:bobwerr}.

\begin{theorem}
For any downward-closed set system and predicted optimal set, \errmech\ with parameters $\gamma = \frac{10(1+\epsilon)}{9\epsilon}$ and $\tau \geq 1$ achieves $(1+\epsilon)$-\tconsistency\ and $O(\frac{\tau}{\epsilon} \log n)$-robustness.
\end{theorem}

For constant $\tau$, the robustness remains asymptotically optimal. Additionally, we note that mechanisms and bounds of this kind are often referred to in the literature as ``error-tolerant'' mechanisms (or algorithms) \textcolor{blue}{add cite}. We thus state the results as a function of the error as well.
\begin{corollary}\label{thm:bobw-err}
    For any downward-closed set system and predicted optimal set, \errmech\ with parameter $\gamma = \frac{10(1+\epsilon)}{9\epsilon}$ and $\tau \geq 1$ achieves an approximation of $(1+\epsilon)\eta$ if $\eta \leq \tau$ and $\left(\frac{2000\tau(1+\epsilon)}{9\epsilon}+1\right)H_n$ otherwise, where $\eta$ is the prediction error defined in~\eqref{def:error}.
\end{corollary}
An immediate open problem would be to quantify how the best possible robustenss changes as we change $\tau$. 


\textcolor{blue}{something other thing I want to say: it is not clear that \sconsistency is always harder, for our problem it is much harder, but for some problems, the trade-offs are the same, which case the error-dependence (smooth) are naturally guaranteed.}




==> 51-conclusions.tex <==
\section{Conclusion and Further Directions}
In this work, we provide the first analysis of clock auctions through the learning-augmented framework. Apart from the standard notion of consistency, we also consider a stronger notion of consistency, which we refer to as \sconsistency. We prove upper and lower bounds on the trade-off between robustness and each of these notions of consistency. Additionally, we observe that the impossibility results regarding the trade-off between \sconsistency\ and robustness also provide insights into the ``cost of smoothness,'' i.e., the robustness that is achievable if we require the performance to degrade smoothly as a function of the prediction error.

In our setting, the achievable trade-off between consistency and robustness and the achievable trade-off between \sconsistency\ and robustness are drastically different. This is in contrast to some other settings (e.g., \cite{ABGOT22,BFGT23, BMS20}), where there is no separation between the two. An interesting open question is to identify which kinds of problems exhibit such separation and which do not. Another type of result currently lacking in the literature is the ``cost of smoothness'', i.e., the best-possible trade-off between good error-dependence and robustness.

To address the limitations of deterministic clock auctions without prior information, we utilize unreliable predictions. Prior work has also explored Bayesian clock auctions using distributional information on bidders' values \cite{FGGS22} and randomized clock auctions to eliminate the need for prior information altogether \cite{CGS22}. Despite the improvements that these alternative approaches have achieved, there remain large gaps. Determining the tight bounds for Bayesian and randomized clock auctions is one of the most compelling open questions in this line of work. More broadly, the compelling properties of clock auctions make them highly suited to practical applications. Thus, further studying their performance in other auction settings (e.g., procurement auctions and double auction settings), potentially augmented with predictions, is an interesting future direction with important implications for ``real-world'' auction implementation.
% One of the most compelling open questions is determining the exact guarantees achievable such clock auctions.  The state-of-the-art guarantees for both Bayesian and randomized auctions are $O(\log \log k)$-approximations where $k$ is the number of maximal feasible sets.  On the other hand, the best known impossibility results are small constants even for general downward-closed feasibility constraints.  This means that, as far as we know, a randomized clock auction can achieve small constant approximation guarantees in highly general settings, whereas deterministic clock auctions (without prior information) can only achieve logarithmic guarantees even in simple settings.  Tightening this gap is a very interesting direction.  More broadly, as we noted earlier, the compelling properties of clock auctions make them highly suited to practical applications, so further studying their performance in other auction settings (e.g., procurement auction and double auction settings) is an interesting future direction that has important implications for ``real-world'' auction implementation.


==> arxiv40-general.tex <==

We first present a strategyproof mechanism that is $1+\epsilon$-consistent and $\theta(\log n)$-robust. 

\begin{theorem}
The BWFCA is $(1+\epsilon)$-consistent and $\theta(\log n)$-robust in any downward-closed set system.
\end{theorem}

\paragraph{The BWFCA mechanism} We modify the water-filling clock auction (WFCA) proposed in \cite{CGS22} as follows: all bidders are initialized to a price of $0$. At each round of the auction, we find the feasible subset of active bidders with the highest revenue (i.e., the highest total sum of clock prices) and let the bidders in that set be ``conditional winner'' in the round. Among the bidders which are not conditional winners, we select the bidder(s) with the lowest price and increase the corresponding price(s) by some small constant $\epsilon$. Compared with the standard WFCA, for bidders in $\pred$, the predicted optimal set, the auction favors them by charging them a price that is $\alpha$ of what they are supposed to be charged in WFCA. \xnote{In addition, the algorithm counts any overlap between the predicted set with other set only to the predicted set, i.e., $F = F \setminus \pred$ for all $F \in \feasible$.} We continue this process until the set of bidders that remain active is feasible.

We now provide some useful observation for the BWFCA mechanism, we first connect the BWFCA mechanism guarantees with the WFCA mechanism guarantees.


\paragraph{The Equivalent Value Boosting Analysis} We construct a modify instance $I'$ given any instance $I$ as follows: Given any instance $I$, and a predicted optimal set $\pred$. For any bidder $i \in \pred$, we change her values from $v_i$ to $v'_i = \alpha\cdot v_i$; for each $F \in \feasible \setminus\{\pred\}$, we let $F' = F \setminus \{\pred\}$. We then perform the WFCA mechanism in the modified instance. It is not hard to see that running BWFCA on the initial instance $I$ is equivalent as running WFCA on the modified instance $I'$, i.e., the bidders will drop out in the same sequence, leading to the same winner set for any instance pairs.\xnote{do we need a proof?} We then show the desired bounds for consistency and robustness using the WFCA guarantees on the modified instance.

\begin{lemma}\label{lem:equivalance}
    Given a instance $I$ and a predicted optimal set $\pred$, let $I'$ be the modified instance described above, then running BWFCA on I and $\pred$ is equivalent as running $WFCA$ on the modified instance $I'$, i.e.,
    $$\text{BWFCA}(I, \pred) = \text{WFCA}(I').$$
\end{lemma}

\begin{theorem}[\cite{CGS22}]\label{thm:wfca} WFCA obtains a $4\log n$-approximation to the optimal social welfare in any downward-closed set system.
\end{theorem}
\xnote{we can show with 1 vs many that this robustness is tight. Not sure if we should include the proof}

We now argue the robustness of the BWFCA with any $\alpha >1$.
\begin{lemma}
BWFCA is $8 \alpha \log n$-robust.
\end{lemma}
\begin{proof}
First note that by Lemma~\ref{lem:equivalance}, it is suffice to consider the set output by WFCA on the modified instance $I'$, let $\opt'$ be the optimal solution for $I'$, We first have that
\begin{align}\label{eq:updatedoptbound}
    v(\opt) \leq 2v'(\opt')
\end{align}
To see this, we consider the following two difference cases: If $v(\pred \cap \opt) \geq \frac{1}{2} \cdot v(\opt)$, we have $$v'(\opt') \geq v'(\pred) \geq v(\pred) \geq \frac{1}{2} \cdot v(\opt),$$ where the third inequality is since the modification only scale up values. Similarly, if $v(\pred \cap \opt) < \frac{1}{2} \cdot v(\opt)$, then we have $$v'(\opt') \geq v'(\opt \setminus \pred) \geq v(\opt \setminus \pred)  \geq \frac{1}{2} \cdot v(\opt).$$
 Let set $M$ be the final set of bidders output by WFCA in instance $I'$, by Theorem~\ref{thm:wfca}, $v'(\opt') \leq 4 \log n v'(M)$. We therefore have
$$v(\opt)  \leq 2v'(\opt')
     \leq 8 \log n v'(M)
    \leq 8 \alpha \log n \cdot  v(M),$$
where the last inequality is due to the definition of the instance modification, i.e., $v'_i \leq \alpha v_i$ for all $i \in M$ \xnote{todo write this out as an observation}.
\end{proof}

\begin{lemma}
BWFCA is $\max\{\frac{4 \log n}{\alpha}, \frac{\alpha}{\alpha - H_{\opt}}\}$-consistent for $\alpha \geq H_{\opt}$.
\end{lemma}
\begin{proof}
 % Recall that the for the consistency case corresponds to the case where the prediction is correct, i.e., $\pred = \opt$. As a consequence, we have $v'(\opt') \geq \alpha v(\opt)$. 
 Again let $M$ to be the output of the WFCA on the modified instance, applying theorem again we get $v'(\opt') \leq 4 \log n  v'(M)$. We now consider the following two cases for $M$.

\paragraph{Case one: $M \not\subseteq \pred$.} If $M \not\subseteq \opt$, we have $v'(M) = v(M)$ since none of the bidder is scaled from the modification. We therefore have 
$$v(\pred) = \frac{v'(\pred)}{\alpha} \leq \frac{v'(\opt')}{\alpha} \leq \frac{4 \log n}{\alpha} v'(M) \leq \frac{4 \log n}{\alpha} v(M),$$
where the first equality is by definition of the modification, the second inequality is by Theorem~\ref{thm:wfca}.
\paragraph{Case two: $M \subseteq \pred$.} To argue that we have enough values in $v(M)$, we will upper bound the value rejected from $\pred$.  
We first note that based on the definition of WFCA, the price posted to the bidders in $\opt$ at any point $t$ is:
\[\frac{\max(p(F'): F' \in \feasible \setminus \{\pred\})}{|\pred_t|},\]
where $\pred_t$ is the set of agent from $\pred$ still in the auction at time $t$ and $p(F)$ is the revenue of set $F$. Let $F^*$ be the set with the highest social welfare excluding $\pred$, i.e., $F^* = \argmax(v'(K): K \in \feasible \setminus \{\opt\})$. 
% Note that $v(S) \leq v(\opt)$.
Now consider all the bidders that are rejected in $\pred$, denoted as $R$, we have:\xnote{maybe the inequality below could be tighter with more refined analysis considering overlapping (for the more general consistency analysis)}
\begin{align*}
    v'(R) &\leq \sum_{i = |\pred| - |R|}^{|\pred|} \frac{\max(p(F'): F' \in \feasible \setminus \{\pred\})}{i} \leq \sum_{i = |\pred| - |R|}^{|\pred|} \frac{\max(v'(F'): F' \in \feasible \setminus \{\pred\})}{i}\\
    &\leq \sum_{i = |\pred| - |R|}^{|\pred|} \frac{v'(F^*)}{i} 
     = \sum_{i = 1}^{|\pred|} \frac{v(F^*)}{i} \leq \sum_{i = 1}^{|\pred|}\frac{v(\opt)}{i} \leq v(\opt)H_{|\pred|}.
\end{align*}
We therefore have:
\[v(M) = v(\pred) - v(R) = v(\pred) - \frac{v'(R)}{\alpha} \geq v(\pred) - \frac{v(\opt)H_{|\pred|}}{\alpha} 
\qedhere\]
% \geq v(\opt) \cdot \left(1 - \frac{H_{|\opt|}}{\alpha}\right)
\end{proof}

\subsection{Impossibility Result}
We now show that $\alpha = $ is the optimal choice of $\alpha$ for BWFCA. In particular, we show that any $\alpha < H_{n-1}$ will lead to $\Omega(\log(n))$ consistency.

\paragraph{Instance} Given some $\alpha < H_{n-1}$, consider the instance with 2 maximal set $A$ $B$, where $B$ has a single agent with value $1$ and $A$ has n-1 agent, and for agent $i \in A$ we have $v(i) = 1/\alpha\cdot i$, therefore we have: 
$$v(A) = \sum_{i \in A}v(i) = \sum_{i \in A} \frac{1}{\alpha \cdot i} = \frac{1}{\alpha}\cdot H_{n-1} >1$$
where the inequality is since $\alpha \leq H_{n-1}$. For the consistency case, we have the prediction set is the optimal set which is $A$. Consider running BWFCA with the given $\alpha$. At any giving point, the revenue we get from set $A$, with the $\alpha$ scaling, is $1$. Using tie breaking (\xnote{we can add $\epsilon$ to avoid the tie breaking}), we can make agent $A$ win with only one item left, leading to an outcome with $1/\alpha$. whereas the optimal solution is $\frac{H_{n-1}}{\alpha}$, leading to a $H_{n-1}$ consistency.

\subsection{$\alpha_k$ type of mechanism?}









